Amortized Noisy Channel Neural Machine Translation

Noisy channel models have been especially effective in neural machine translation (NMT). However, recent approaches like "beam search and rerank" (BSR) incur significant computation overhead during inference, making real-world application infeasible. We aim to study if it is possible to build an amortized noisy channel NMT model such that when we do greedy decoding during inference, the translation accuracy matches that of BSR in terms of reward (based on the source-to-target log probability and the target-to-source log probability) and quality (based on BLEU and BLEURT). We attempt three approaches to train the new model: knowledge distillation, one-step-deviation imitation learning, and Q learning. The first approach obtains the noisy channel signal from a pseudo-corpus, and the latter two approaches aim to optimize toward a noisy-channel MT reward directly. For all three approaches, the generated translations fail to achieve rewards comparable to BSR, but the translation quality approximated by BLEU and BLEURT is similar to the quality of BSR-produced translations. Additionally, all three approaches speed up inference by 1-2 orders of magnitude.

==> misc.tex <==




INTRO


% \hh{Right now the three approaches sound rather arbitrary. Maybe say that your goal is to optimize the reward, i.e. the forward and reverse probabilities. Then you can consider BSR as the "oracle", and call KD behavior cloning, so that the three methods have increasingly more exploration when optimizing the reward.}




BACKGROUND


% In particular, greedy decoding from $p_\theta$ is as follows: to generate the $t$-th token, $\hat{y}_t = \argmax_{v\in \mathcal{V}} p_\theta(v\mid \vy_{<t}, \vx)$, where $\mathcal{V}$ is the target-language vocabulary\hh{Probably don't need to explain what greed decoding is. You can both are approximate search methods to find the highest scoring translation.}. % Beam search with beam size $b$ from $p_\theta$ starts from a set of empty prefixes; at each time step $t$, we expand each prefix (in the prefix set) with each possible token, then select the $b$ best expanded prefixes (corresponding to highest prefix probability), to form the the new set of prefixes.






% For instance, if a translation system is put online for an indefinite amount of time, then in the long run, better test-time efficiency could save a considerable amount of energy and cost\hh{This high-level motivation should be in the intro.}.  % In addition, if a translation system is run offline on a mobile device, then a highly inefficient reranking approach may be infeasible.  % The efficiency for doing CPU-only inference without batch parallelization (when decoding the large beam and feeding the large beam to the reverse models) may hurt to a great degree, with a slow noisy-channel NMT inference algorithm. 
% 





APPROACHES



% Unlike common cases where the teacher network is stronger (e.g., the teacher network has a larger number of parameters, or the teacher network is autoregressive whereas the student network is non-autoregressive), here, the teacher network $p_f$ and the student network $p_d$ have the same architecture. 
% \hh{Unclear what's the takeaway from this paragraph. Also the teacher is BSR($p_f$).}







% Inspired by ENGINE \citep{tu-etal-2020-engine}, which trains a non-autoregressive inference network (student) using an autoregressive scoring function (teacher), we propose the following adaptation in the context of noisy-channel NMT. Like \citeauthor{tu-etal-2020-improving}, we define an autoregressive inference network $A_\phi$ (with the same architecture as $p_f$) whose input is a sentence $\vx$ and whose output is a translation $\vy$. 

% $A_\phi$ takes in only one argument: a source sentence $\vx$. 
% $A_\phi(\vx) = [\hat{y}_1, \hat{y}_2, \dots, \hat{y}_T]$ where 
% \begin{align}
%     \vz_t &= p^{ENG}_\phi(\cdot \mid \vx, \hat{\vy}_{<t}) \nonumber \\ 
%     \hat{y}_t &= \argmax \vz_t \nonumber \\
%     \hat{\vy}_{<1} &= \varnothing \nonumber
% \end{align} 
% $A_\phi(\vx)$ is trained with the goal that 
% \begin{align}
%     A_\phi(\vx)\approx \argmin_{\vy'} E_\theta(\vx, \vy').
% \end{align} 

% \paragraph{Energy.} In the context of noisy-channel NMT:
% \begin{align}
%     & E_\theta(\vx, \vz) = \sum_{t=1}^{T} e_t^f (\vx, \vz) + \gamma \sum_{t'=1}^{|\vx|} e_{t'}^r (\vx, \vz),  \label{eq:energy-ncmt}
% \end{align}
% where $\vz=(\vz_1, \vz_2, \dots, \vz_T)$ and $\vz_i \in \mathbb{R^{|\mathcal{V}|}}$. 

% % Let $O=\mathrm{softmax}$.\footnote{We could attempt other operators including Gumbel-softmax and straight-through, but we omit them in this work, given that it is not central to our thesis. Refer to \citet{gu2018neural} and \citet{tu-etal-2020-engine} for details on more potential operators.} 
% In Eq.~(\ref{eq:energy-ncmt}), we define the forward sub-energy $e_t^f$ as follows:\footnote{Suppose we  compute $p_\theta^f(\cdot \mid y_1, y_2, \dots, y_{t-1}, \vx)$ where $y_i$'s correspond to token ids of a partial translation in the target language, then in our implementation, we first look up the $y_i$-th row of the embedding matrix $E_{emb}$ and use this row to represent $y_i$. Equivalently, we can use the product $\mathrm{onehot}(y_i)^\top E_{emb} $ to represent $y_i$. In the case of the ENGINE sub-energy $e_t^f$, we can use $O(\vz_i)^\top E_{emb}$ to represent $\vz_i$. Both $\mathrm{onehot}(y_i)$ and $O(\vz_i)$ are probability distributions with $|\mathcal{V}|$ dimensions.} 
% \begin{align}
%     & e_t^f (\vx, \vz) = - \vz_t^\top \log p_\theta^f (\cdot \mid \vz_1, \dots \vz_{t-1}, \vx). \nonumber 
% \end{align}
% We define the reverse sub-energy as follows:
% \begin{align}
%     & e_t^r (\vx, \vz) = - \mathrm{onehot}(\vx_t)^\top \nonumber \\ 
%     & \qquad \log p_\theta^r (\cdot \mid \vx_{<t}, \vz_1, \dots \vz_{T}). \nonumber
% \end{align}

% \paragraph{Training objective.} To train $A_\phi(\vx)$ so that $A_\phi(\vx)$ achieves the approximation shown in Eq.~(\ref{eq:energy-ncmt}), we optimize the following:
% \begin{align}
%     {\phi^\ast} = \argmin_\phi \sum_{(\vx,\vy) \in \mathcal{D}} E_\theta(\vx, A_\phi(\vx)).
% \end{align} 

% \paragraph{Inference.} During inference, we do inference using $A_\phi (\vx)$ directly. Specifically, we do \emph{greedy decoding}:
% \begin{align}
%     \hat{y}_t = \argmax_{v \in \mathcal{V}} p^{ENG}_\phi (v \mid \vy_{<t}, \vx)
% \end{align}


% \subsection{Approach 2: One-step deviation imitation 








% 

% Let $O=\mathrm{softmax}$.\footnote{We could attempt other operators including Gumbel-softmax and straight-through, but we omit them in this work, given that it is not central to our thesis. Refer to \citet{gu2018neural} and \citet{tu-etal-2020-engine} for details on more potential operators.} 
% Observe that the differences between the sub-energies and Eq.~(\ref{eq:imit}) are as follows. First, in $e_t^f$, the prefixes used in $p^f_\theta$ are distributions instead of tokens which can also be interpreted as one-hot distributions, and similarly for $e_t^r$. Second, we use examples greedily decoded from the current model $A_\phi$ instead of fixed examples from an existing dataset. \pang{Edit.} 





% \hh{If someone doesn't know Q-learning, this short description is not helpful. If someone does know Q-learning, this is redundant. So I'd remove it.}In short, given a trajectory $(\vx, \vy, \vr)$, at time-step $t<T$, we want the scalar $Q(s_t, a_t)$ to be close to the sum of the $t$-th step reward % (i.e., the forward log probability $\log p_f(a_t \mid \vy_{<t}, \vx)$) 
% and the \textit{most optimistic} future return, % for steps $\geq t+1$
% had we taken action $a_t$ at time-step $t$. At time-step $T$, we want $Q(s_T, a_T)=Q(({\vy}_{<T}, \vx), \langle \text{eos} \rangle)$ to be close to $r_T$, as defined in Eq.~(\ref{eq:q-reward}). 

% Thus, the inference speed of $Q$ and that of $p_f$ are the same. 










ALGO



        % \quad \textbullet\ if $t<T$, then $R_t = {\log p_f(y_t|{\vy}_{<t}, \vx)} + \max_{v} Q_\phi'([{\vy}_{<(t+1)};v], \vx);$\\
        % \quad \textbullet\ if $t=T$, then $R_t = \log p_f(y_t|{\vy}_{<t}, \vx) + \lambda \cdot {\log p_r(\vx|\vy)}.$\\

        % Update $Q_\phi$ according to the following objective:
        % $\argmin_\phi \left[ Q_\phi([{\vy}_{<t}; y_t], \vx) - R_t \right]^2$.\\
        
        













% \paragraph{Language model score.} We also investigate the fluency of translations, approximated by the average token perplexity scored by GPT-2 \citep{radford2019language}. Given that the average perplexity may be very large for short sequences,\footnote{The probability (scored by GPT-2) for the first token is usually very small.} we only score translations whose corresponding source sequences have length larger than 20; there are 3,581 such sequences. We see that the average perplexity for the reference translations are much lower than the rest. $Q$-generated translations have the largest average perplexity. If we have access to a high-quality language model (potentially trained on a large corpus in the target language), then we can add the language modeling scores to the reward function in Eq.~(\ref{eq:reward}).
% Using a revised reward function may improve the fluency of $Q$.\footnote{Recall that we skipped the language modeling term in this paper, given that the goal is orthogonal to our thesis.}







% \subsection{Discussion on Reward vs. BLEU}

% \begin{figure}[t!]
%      \centering
%          \includegraphics[width=0.9\columnwidth]{figs/sentence_bleu_reward_f.pdf}
%     \caption{Sentence-level sacreBLEU vs. total reward. The sacreBLEU uses (default) exponential smoothing to avoid zero BLEUs. ``$p_f$ beam5'' refers to beam search decoding from $p_f$; ``rerank'' refers to BSR; the other three approaches refer to approaches 1, 2, 3 (Section~\ref{sec:methods}), respectively. We see that lower rewards usually leads to smaller BLEU; larger rewards can lead to either small or large BLEU scores.}
%     \label{fig:sentence_bleu_reward}
% \end{figure}


% \begin{figure*}[t]
%      \centering
%      \begin{subfigure}[t]{0.31\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/sentence_bleu_reward_f.pdf}
%          \caption{Sentence-level BLEU vs. forward reward. We see that lower rewards usually lead to smaller BLEU; larger forward rewards can lead to either small or large BLEU scores.}
%          \label{fig:sentence_bleu_reward_f}
%      \end{subfigure}
%      \quad
%      \begin{subfigure}[t]{0.31\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/sentence_bleu_reward_r.pdf}
%          \caption{Sentence-level BLEU vs. reverse reward. We see that lower rewards usually lead to smaller BLEU; larger reverse rewards can lead to either small or large BLEU scores.}
%          \label{fig:sentence_bleu_reward_r}
%      \end{subfigure}
%      \quad
%      \begin{subfigure}[t]{0.31\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/sentence_two_rewards.pdf}
%          \caption{Sentence-level reverse reward vs. forward reward. A large number of translations have large forward rewards but small reverse rewards, and vice versa.}
%          \label{fig:sentence_two_rewards}
%      \end{subfigure}

%     \caption{
%         Relationships among forward reward, reverse reward, and BLEU. We use sacreBLEU for the BLEU computation, and it uses (default) exponential smoothing to avoid zero BLEUs. ``$p_f$ beam5'' refers to beam search decoding from $p_f$; ``rerank'' refers to BSR; the other three approaches refer to approaches 1, 2, 3 (Section~\ref{sec:methods}), respectively. 
%     }
%     \label{fig:sentence_bleu_rewardf_rewardr}
        
% \end{figure*}

% We have seen in Table~\ref{tab:main} that ``greedy decoding from $p_f$'' and ``beam search from $p_f$'' have the smallest reverse rewards (not considering the reference data\footnote{We hypothesize that given that there may be ``outlier'' translations with rare tokens, non-standard grammars, and incorrect tokens in the original corpus, it is hard for $p_f$ and $p_r$ to assign high probabilities to them.}), and the BLEU scores of these two approaches are bottom-ranked too. 
% This observation motivates us to further investigate the relationship among BLEU, forward reward, and reverse reward.  


% \paragraph{Sentence-level BLEU vs. reward.}

% Figures~\ref{fig:sentence_bleu_reward_f} and \ref{fig:sentence_bleu_reward_r} show the sentence-level BLEU vs. forward reward and BLEU vs. reverse reward for sequences whose length is in $[20,25]$ for the IWSLT'14 De-En dataset.\footnote{We only include sequences with a certain length in case the length confounds our analysis. The trend for other length buckets (assuming there are enough translations in the bucket) is similar.} For clarity, we only include five systems.  
% We see that given a sequence, if the forward (or reverse) reward of the sequence is small then it is unlikely to have a large BLEU. If the forward (or reverse) reward of the sequence is large then it could, but not necessarily, have a large BLEU. 


% One may claim that the high-reward sequences are of high quality, but given the diversity of reference translations, BLEU may be inaccurate. We therefore plot BLEURT \citep{sellam-etal-2020-bleurt} vs. reward in Appendix~\ref{app:analysis} and find a similar trend to Figure~\ref{fig:sentence_bleu_reward}. 


% \begin{figure}[ht!]
%      \centering
%          \includegraphics[width=0.98\columnwidth]{figs/system_bleu_reward.pdf}
%     \caption{System-level sacreBLEU vs. reward. Left: IWSLT'14 De-En. Right: WMT'16 Ro-En.}
%     \label{fig:system_bleu_reward}
% \end{figure}


% \paragraph{Sentence-level forward reward vs. reverse reward.}

% Figure~\ref{fig:sentence_two_rewards} shows the reverse rewards $\log p_r (\vx \mid \vy)$ vs. the forward rewards $\log p_f(\vy \mid \vx)$ for translations whose length is in $[20,25]$. The plot for all lengths are in Appendix~\ref{app:analysis}. We see that a large number of sentences have large forward rewards but small reverse rewards, and vice versa. Therefore, including the reverse reward (i.e., channel reward) is still justified.  


% \paragraph{System-level BLEU vs. reward.}

% From Table~\ref{tab:main}, we see that generally, a higher reward correspond to a larger BLEU. However, the BLEUs and median rewards of the reference translations have the opposite trend: the BLEUs are the largest (100) but the rewards are the lowest. We hypothesize that given that there may be ``outlier'' translations with rare tokens, non-standard grammars, and incorrect tokens in the original corpus, it is hard for $p_f$ and $p_r$ to assign high probabilities to them. Should we still optimize toward the reward shown in Eq.~(\ref{eq:reward}) in NMT systems? We see from Table~\ref{tab:main} and the recent top-performing systems \citep{ng-etal-2019-facebook,tran2021facebook} that using the noisy channel objective is still effective at improving translation quality empirically.





















% \begin{table}[ht!]
% \setlength{\tabcolsep}{3.3pt}
% \centering
% \small
% % \fontsize{11}{13.2}\selectfont 
% \begin{tabular}{>{\hangindent=0.6em\hangafter=1}m{2.8cm}ccccc}
%     \toprule
%     \noalign{\smallskip}
%     & \makecell[c]{length \\ mean} & \makecell[c]{num unique \\ tokens} & \makecell[c]{token rep \\ (\%)}   \\
%     \midrule
%     $p_f$ (greedy decoding) & 28.17 & 6957 & 4.18 \\
%     $p_f$ (beam search) & 28.21 & 6970 & 4.08 \\
%     {beam search \& rerank} & 28.31 & 7092 & 3.95 \\
%     \specialrule{.2pt}{1pt}{1pt}

%     $p_{\mathrm{KD}/nc}$ (approach 1) & 28.15 & 6953 & 4.03 \\ 
%     $A$ (approach 2) & 28.19 & 6959 & 3.92 \\
%     $Q$ (approach 3) & 27.88 & 6894 & 4.85 \\  % three runs (34.54, 34.67, 34.58)
%     \specialrule{.2pt}{1pt}{1pt}

%     reference data & 28.48 & 7201 & 3.59 \\
% \bottomrule
% \end{tabular}
% \caption{Analyses of WMT'16 Ro-En translations on the development set.
% }
% \label{tab:analysis}
% \end{table}






% \paragraph{Word frequencies.} The number of unique tokens used in the reference data is the largest. In fact, the number of tokens that have frequency in $[1, 20]$, $[21, 40]$, $[41, 60]$, $[61, 80]$, $[81, 100]$, $[101, \infty)$ are always larger in reference translations, for each bucket, compared to each of the other systems. For the other models, there is no discernible differences in terms of the number of tokens in each bucket.  



% We first quickly examine two simple properties of generations: the length and lexical diversity by the number of unique tokens. Based on Table~\ref{tab:analysis}, we see that the reference translations and BSR-generated translations are longest, and they have the largest number of unique tokens.




% \paragraph{Coefficient for the reverse reward.} The coefficient $\gamma$ is tuned on the dev set BLEU score using the BSR approach, and for approaches 1-3, we use this same $\gamma$. In BSR, given that the beam size (50--100) is small compared to the combinatorially large number of possible sentences, we are guaranteed to have sequences with large forward rewards $p(\vy \mid \vx)$. If we simply optimize our reward $p(\vy \mid \vx) + \gamma p(\vx \mid \vy)$, then it is possible that approaches 2-3 produce translations that have a much lower forward rewards compared to translations produced by BSR. Therefore, during optimization using approach 2/3, it may be help to reduce $\gamma$. 

















% However, the periodic updates will lead to slower propagation of the newly updated rewards, especially the right-most sparse channel rewards in the Markov chain. In fact, if there are $T$ states in the Markov chain and we update $Q'$ once every $K$ steps, then it would take at least $KT$ steps for an updated sparse channel reward to propagate to the earliest time-step. Reducing $K$ may lead to training instabilities, but having a large $K$ will slow down convergence. 
% Therefore, one possible direction involves exploring non-target-network approaches like using functional regularization \citep{piche2021beyond}, which leads to more efficient learning. Other possible directions to improve learning efficiency from the sparse rewards include R-learning \citep{mahadevan1996average} as well as investigating other strategies to distribute the sparse rewards to earlier in the sequence. 










APPENDIX 




% Let $Q_\phi: \mathcal{S} \times \mathcal{V} \to \mathbb{R}^{|\mathcal{V}|}$ be the optimal action-value function with parameter $\phi$ such that $Q_\phi((\vy_{<t}, \vx), v) =  \max_{\pi} \sum_{t'=t}^\infty r_{t'}$, which is the maximum return (i.e., the maximum of the sum of future reward with discount rate 1) achievable by following any strategy \textit{after} seeing a state $(\vy_{<t}, \vx)$ and taking an action $v$, where $\pi$ is a policy that maps states to actions. 
% % 
% We also denote this scalar using the notation $Q_\phi([\vy_{<t}; v], \vx)$. We may omit the subscript $\phi$ for simplicity. 

% , where $[\vy_{<t}; v]$ represents the concatenation of prefix $\vy_{<t}$ and token $v$.
% Moreover, we use $Q^{\mathcal{V}} (\vy_{<t}, \vx) \in \mathbb{R}^{\mathcal{|V|}}$ to denote the vector containing every $Q^v(\vy_{<t}, \vx)$. 

% %The stochastic policy $\pi$ maps the state to a probability distribution over the action space $\gV$:
% $\pit(a_t\mid s_t) = \pt(a_t\mid \vy_{0:t-1}, \vx)$. 








% \paragraph{More Discussion on Models}







% \section{More Details on Analysis}
% \label{app:analysis}


% \paragraph{Boxplots on length of translations.}

% \begin{figure}[ht!]
%      \centering
%          \includegraphics[width=\columnwidth]{figs/all_len.pdf}
%     \caption{Lengths of generations (based on the dev set) from different systems.}
%     \label{fig:all_len}
% \end{figure}


% Section~\ref{sec:analysis-translations} includes an analysis of lengths of translations generated by different systems. Figure~\ref{fig:all_len} shows the box plot. We see that the median and Q3 for the reference translations are larger than those by other systems. $Q$ produces a translation that is the longest among all translations by all systems, and we have verified that the translation includes lots of repetitions. For the non-reference translations, there is no other discernible differences in terms of length. 



% % \paragraph{Sentence-level BLEU vs. reward.}


% % \begin{figure}[t]
% %      \centering
% %          \includegraphics[width=0.9\columnwidth]{figs/sentence_bleu_reward_all_len.pdf}
% %     \caption{Sentence-level BLEU vs. reward. }
% %     \label{fig:sentence_bleu_reward_all_len}
% % \end{figure}


% % Recall that in Figure~\ref{fig:sentence_bleu_reward}, we only include sequences with a certain length (between 20 and 25, inclusive) in case the length confounds our analysis. The plot for all length buckets is shown in Figure~\ref{fig:sentence_bleu_reward_all_len}. We have clipped a few outliers with very small rewards.




% % \paragraph{Sentence-level BLEURT vs. reward.}

% % \begin{figure}[t]
% %      \centering
% %          \includegraphics[width=0.9\columnwidth]{figs/sentence_bleurt_reward.pdf}
% %     \caption{Sentence-level BLEURT vs. reward. }
% %     \label{fig:sentence_bleurt_reward}
% % \end{figure}

% % Recall that in Figure~\ref{fig:sentence_bleu_reward}, one hypothesis that the high-reward sequences are good, but cannot be scored high by BLEU. We therefore plot BLEURT \citep{sellam-etal-2020-bleurt} vs. reward in Appendix~\ref{app:analysis}. For BLEURT, we use BLEURT-base. Given that it is possible for BLEURT to achieve scores smaller than 0 or larger than 1, we assign the score to be 0 if the BLEURT prediction is smaller than 0, and assign the score to be 1 if the BLEURT prediction is larger than 1. We find that the trend is similar to Figure~\ref{fig:sentence_bleu_reward}. 





% \paragraph{Reverse reward vs. forward reward.}

% \begin{figure}[ht!]
%      \centering
%          \includegraphics[width=0.98\columnwidth]{figs/sentence_two_rewards_all_len.pdf}
%     \caption{Sentence-level reverse reward vs. forward reward for all length buckets.}
%     \label{fig:sentence_two_rewards_all_len}
% \end{figure}

% Recall that in \ref{fig:sentence_two_rewards}, the plot only includes translations with length between 20 and 25 (inclusive). Figure~\ref{fig:sentence_two_rewards_all_len} shows reverse vs. forward rewards for translations of all lengths. A few outliers are truncated from the figure. We can see that a large number of translations have large forward rewards but small reverse rewards, or large reverse rewards but small forward rewards. 


==> table_misc.tex <==











% \begin{table*}[ht!]
% \setlength{\tabcolsep}{2.4pt}
% \centering
% \small
% \begin{tabular}{>{\hangindent=0.9em\hangafter=1}m{3.2cm}ccccccccccc}
%     \toprule
%     & \multicolumn{3}{c}{IWSLT14 De-En} & & \multicolumn{3}{c}{WMT16 Ro-En} & & \multicolumn{3}{c}{WMT14 De-En} \\
%     \cline{2-4} \cline{6-8} \cline{10-12}
%     \noalign{\smallskip}
%     & \makecell[c]{$b$} & \makecell[c]{fwd reward \\ mean (std)} & \makecell[c]{rvs reward \\ mean (std)} &  & $b$ & \makecell[c]{fwd reward \\ mean (std)} & \makecell[c]{rvs reward \\ mean (std)} & & $b$ & \makecell[c]{fwd reward \\ mean (std)} & \makecell[c]{rvs reward \\ mean (std)}  \\
%     \midrule
%     $p_f$  & 1 & -9.1 {\scriptsize (7.7)} & -35.4 {\scriptsize (39.9)} & & 1 & -9.5 {\scriptsize (11.5)} & -41.0 {\scriptsize (50.1)} & & 1 & -10.9 {\scriptsize (6.3)} & -31.5 {\scriptsize (24.6)} \\
%     $p_f$  & 5  & -8.6 {\scriptsize (7.0)} & -34.2 {\scriptsize (38.5)} &  & 5 & -9.0 {\scriptsize (8.5)} & -40.2 {\scriptsize (48.2)} & & 7 & -10.4 {\scriptsize (5.5)} & -29.9 {\scriptsize (21.5)} \\
%     {beam search and rerank} & 100 & -9.4 {\scriptsize (6.8)} & -25.7 {\scriptsize (32.5)} & & 100  & -9.9 {\scriptsize (6.0)} & -29.7 {\scriptsize (41.9)} & & 50 & -10.7 {\scriptsize (5.3)} & -23.6 {\scriptsize (16.3)}\\
%     \specialrule{.2pt}{1pt}{1pt}

%     $p_{KD/beam}$ trained by $(X, \widetilde{Y}_{beam})$ & {1}  & -13.3 {\scriptsize (13.4)} & -31.6 {\scriptsize (35.2)} & & 1  & -17.0 {\scriptsize (17.4)} & -38.9 {\scriptsize (49.0)}  & & 2 & -14.4 {\scriptsize (8.8)} & -30.1 {\scriptsize (25.0)} \\ 
%     \specialrule{.2pt}{1pt}{1pt}

%     $p_{KD/nc}$ trained by $(X, \widetilde{Y}_{NC})$ (approach 1) & {1} & -13.8 {\scriptsize (13.9)} & -28.0 {\scriptsize (32.7)} & & 5  & -16.7 {\scriptsize (14.9)} & -33.8 {\scriptsize (44.5)} & & 1  & -14.8 {\scriptsize (9.1)} & -24.0 {\scriptsize (16.7)} \\ 
%     $A$ (approach 2) & {1} & -13.4 {\scriptsize (13.3)} & -28.0 {\scriptsize (32.8)} & & 6 & -9.5 {\scriptsize (8.5)} & -37.2 {\scriptsize (45.3)} & & 5 & -11.3 {\scriptsize (6.0)} & -26.1 {\scriptsize (17.7)} \\
%     $Q$ (approach 3) & {1} & -13.7 {\scriptsize (21.4)} & -29.9 {\scriptsize (35.1)} & & 1  &  -13.8 {\scriptsize (20.4)} & -37.3 {\scriptsize (47.9)} & & 1  &  -13.0 {\scriptsize (10.2)} & -28.1 {\scriptsize (27.9)}\\ 
%     \specialrule{.2pt}{1pt}{1pt}

%     reference data & -- & -38.8 {\scriptsize (39.7)} & -45.2 {\scriptsize (46.6)} & & -- &  -55.3 {\scriptsize (51.1)} & -59.0 {\scriptsize (54.2)} & & -- & -36.8 {\scriptsize (24.4)} & -36.8 {\scriptsize (23.0)}  \\
% \bottomrule
% \end{tabular}
% \caption{Test set forward and reverse rewards for translations generated by different models (using random seed 1 for each row). In the second column, $b$ refers to beam size during inference; $b$'s for $p_{\mathrm{KD}}, A, Q$ are tuned according to dev set median reward. Recall that $\gamma$ is the coefficient of the reverse reward, when computing the total reward in Eq.~(\ref{eq:reward}); it is tuned on dev set BLEU using ``beam search and rerank.'' $\gamma=0.9$ for IWSLT14 De-En; $\gamma=0.5$ for WMT16 Ro-En and WMT14 De-En.
% }
% \label{tab:main}
% \end{table*}














% \begin{table}[ht!]
% \setlength{\tabcolsep}{2.1pt}
% \centering
% \small
% \begin{tabular}{>{\hangindent=0.9em\hangafter=1}m{2.8cm}cccccccccc}
%     \toprule
%     & \makecell[c]{IWSLT14 \\ De-En} & \makecell[c]{WMT16 \\ Ro-En} & \makecell[c]{WMT14 \\ De-En}   \\
%     % \noalign{\smallskip}
%     \midrule
%     $p_f$ (greedy decoding)  & 33.65 {\scriptsize (0.06)} & 33.23 {\scriptsize (0.14)} & 30.39 {\scriptsize (0.13)}  \\
%     $p_f$ (beam search) & 34.54 {\scriptsize (0.08)} & 33.98 {\scriptsize (0.15)} & 31.80 {\scriptsize (0.07)} \\
%     {beam search \& rerank} & {35.43} {\scriptsize (0.06)} & \textbf{34.61} {\scriptsize (0.14)} & \textbf{32.18} {\scriptsize (0.19)}   \\
%     \specialrule{.2pt}{1pt}{1pt}

%     $p_{KD/beam}$ &  34.80 {\scriptsize (0.11)} & 33.22 {\scriptsize (0.09)} & 31.38 {\scriptsize (0.11)} \\ % & -56.0/-36.0/-19.0 \\
%     \specialrule{.2pt}{1pt}{1pt}

%     $p_{KD/nc}$ (approach 1) & 35.39 {\scriptsize (0.04)} & 34.31 {\scriptsize (0.20)} & 31.77 {\scriptsize (0.06)}\\ 
%     $A$ (approach 2) & \textbf{35.59} {\scriptsize (0.11)} & {34.30} {\scriptsize (0.11)} & {31.36} {\scriptsize (0.16)} \\
%     $Q$ (approach 3) & 34.62 {\scriptsize (0.07)} & 33.76 {\scriptsize (0.27)} & 30.62 {\scriptsize (0.36)} \\ 

% \bottomrule
% \end{tabular}
% \caption{Test set BLEU (the average and the standard deviation of three runs using different random seeds). All the BLEU scores in this paper are computed by SacreBLEU \citep{post-2018-call} after detokenizing all the translations. 
% }
% \label{tab:main-bleu}
% \end{table}




% \begin{table}[ht!]
% \setlength{\tabcolsep}{1.5pt}
% \centering
% \small
% % \fontsize{11}{13.2}\selectfont 
% \begin{tabular}{>{\hangindent=1.0em\hangafter=1}m{1.7cm}ccc}
%     \toprule
%     & \multicolumn{3}{c}{WMT14 De-En} \\
%     \cline{2-4} 
%     \noalign{\smallskip}
%      & $b$  & \makecell[c]{forward reward \\ Q1/median/Q3}  & \makecell[c]{reverse reward \\ Q1/median/Q3}  \\
%     \midrule
%     $p_f$ & 1 &  -34.5/-23.2/-14.7 & -9.8/-26.0  \\
%     $p_f$ & 7 &  -33.0/-22.3/-14.4 & -9.5/-25.4  \\
%     {beam search \& rerank} & 50 & -29.4/-20.2/-13.1 & -9.9/-20.1  \\
%     \specialrule{.2pt}{1pt}{1pt}

%     $p_{KD/beam}$ & 1 & -37.9/-25.0/-15.7 & -12.8/-24.1   \\
%     $p_{KD/nc}$  & 1 & -35.1/-23.6/-14.8 & -12.9/-11.9  \\  
%     $A$ & \\
%     $Q$ & \\  
%     \specialrule{.2pt}{1pt}{1pt}

%     reference & n/a & &  \\
% \bottomrule
% \end{tabular}
% \caption{Test set rewards for WMT14 De-En. Please refer to Table~\ref{tab:main} for the detailed caption. This table is created given space constraints in Table~\ref{tab:main}.
% }
% \label{tab:main-wmt14}
% \end{table}









% \begin{table*}[ht!]
% \setlength{\tabcolsep}{2.1pt}
% \centering
% \small
% \begin{tabular}{>{\hangindent=0.9em\hangafter=1}m{3.3cm}cccccccccc}
%     \toprule
%     & \multicolumn{4}{c}{IWSLT14 De-En} & & \multicolumn{4}{c}{WMT16 Ro-En}  \\
%     \cline{2-5} \cline{7-10}
%     \noalign{\smallskip}
%     & \makecell[c]{$b$} & \makecell[c]{reward ($\uparrow$) \\ Q1/median/Q3} & \makecell[c]{fwd/rvs \\ reward ($\uparrow$)} & BLEU ($\uparrow$) &  & $b$ & \makecell[c]{reward ($\uparrow$) \\ Q1/median/Q3} & \makecell[c]{fwd/rvs \\ reward } & BLEU ($\uparrow$) \\
%     \midrule
%     $p_f$ & {1} &  -54.1/-28.6/-13.9 & -7.0/-23.8 & 33.65 {\scriptsize (0.06)} & & 1  & -37.7/-24.2/-13.8 & -7.9/-31.5 & 33.23 {\scriptsize (0.14)} \\
%     $p_f$  & 5  & -52.6/-28.0/-13.4 & \textbf{-6.8}/-23.2 & 34.54 {\scriptsize (0.08)} & & 5  & -37.1/-23.7/-13.6 & \textbf{-7.7}/-31.1 & 33.98 {\scriptsize (0.15)} \\
%     {beam search \& rerank} & 100 & \textbf{-42.5}/\textbf{-22.2}/\textbf{-11.2} & -8.2/\textbf{-15.5} & {35.43} {\scriptsize (0.06)} & & 100  & \textbf{-31.7}/\textbf{-20.1}/\textbf{-11.8} & -9.1/\textbf{-22.1} & \textbf{34.49} {\scriptsize (0.35)}  \\
%     \specialrule{.2pt}{1pt}{1pt}

%     $p_{KD/beam}$ trained by $(X, \widetilde{Y}_{beam})$ & {1}  & -55.2/-29.1/-14.0 & -9.4/-21.4 & 34.80 {\scriptsize (0.11)}& & 1  & -46.3/-29.7/-15.7 & -13.5/-30.6 & 33.24 {\scriptsize (0.06)} \\ % & -56.0/-36.0/-19.0 \\
%     $p_{KD/nc}$ trained by $(X, \widetilde{Y}_{NC})$ (approach 1) & {1} & -51.6/-26.9/-13.1  & -9.7/-18.4 & 35.39 {\scriptsize (0.04)} & & 5  & -42.7/-27.2/-14.7 & -13.4/-26.3 & 34.31 {\scriptsize (0.20)}\\ 
%     $A$ (approach 2) & {1}  & -50.7/-26.5/-12.8 & -9.7/-18.2 & \textbf{35.57} {\scriptsize (0.15)} & & 5 & -35.4/-23.4/-13.3 & -8.1/-29.6 & {34.15} {\scriptsize (0.18)} \\
%     $Q$ (approach 3) & {1} & -53.2/-28.0/-13.4 & -9.4/-20.0 & 34.62 {\scriptsize (0.07)} & & 1  & -38.1/-24.0/-13.7 & -9.9/-28.3 & 33.76 {\scriptsize (0.27)} \\ 
%     \specialrule{.2pt}{1pt}{1pt}

%     reference data & n/a & -106.2/-58.0/-28.5 & -27.9/-32.4 & n/a & & n/a & -124.4/-79.6/-43.4 & -44.0/-48.6 & n/a \\
% \bottomrule
% \end{tabular}
% \caption{Test set BLEU (the average and the standard deviation of three runs using different random seeds) and rewards for translations generated by different models (using random seed 1 for each row), for IWSLT14 De-En and WMT16 Ro-En. Due to space constraints, the results for WMT14 De-En are included in Table~\ref{tab:main-wmt14}. In the second column, $b$ referes to beam size during inference; $b$'s for $p_{\mathrm{KD}}, A, Q$ are tuned according to dev set median reward. All the BLEU scores in this paper are computed by SacreBLEU \citep{post-2018-call} after detokenizing all the translations. For each set of translations, we report the Q1 (first quartile), median, and Q3 (third quartile) of the rewards defined in Eq.~(\ref{eq:reward}); we also report the median forward/reverse rewards. 
% }
% \label{tab:main}
% \end{table*}




% \begin{table}[ht!]
% \setlength{\tabcolsep}{1.5pt}
% \centering
% \small
% % \fontsize{11}{13.2}\selectfont 
% \begin{tabular}{>{\hangindent=1.0em\hangafter=1}m{1.7cm}ccc}
%     \toprule
%     & \multicolumn{3}{c}{WMT14 De-En} \\
%     \cline{2-4} 
%     \noalign{\smallskip}
%      & $b$  & \makecell[c]{forward reward \\ Q1/median/Q3}  & \makecell[c]{reverse reward \\ Q1/median/Q3}  \\
%     \midrule
%     $p_f$ & 1 &  -34.5/-23.2/-14.7 & -9.8/-26.0  \\
%     $p_f$ & 7 &  -33.0/-22.3/-14.4 & -9.5/-25.4  \\
%     {beam search \& rerank} & 50 & -29.4/-20.2/-13.1 & -9.9/-20.1  \\
%     \specialrule{.2pt}{1pt}{1pt}

%     $p_{KD/beam}$ & 1 & -37.9/-25.0/-15.7 & -12.8/-24.1   \\
%     $p_{KD/nc}$  & 1 & -35.1/-23.6/-14.8 & -12.9/-11.9  \\  
%     $A$ & \\
%     $Q$ & \\  
%     \specialrule{.2pt}{1pt}{1pt}

%     reference & n/a & &  \\
% \bottomrule
% \end{tabular}
% \caption{Test set rewards for WMT14 De-En. Please refer to Table~\ref{tab:main} for the detailed caption. This table is created given space constraints in Table~\ref{tab:main}.
% }
% \label{tab:main-wmt14}
% \end{table}
